Data Migration using Datalog Program Synthesis

This paper presents a new technique for migrating data between different schemas. Our method expresses the schema mapping as a Datalog program and automatically synthesizes a Datalog program from simple input-output examples to perform data migration. This approach can transform data between different types of schemas (e.g., relational-to-graph, document-to-relational) and performs synthesis efficiently by leveraging the semantics of Datalog. We implement the proposed technique as a tool called Dynamite and show its effectiveness by evaluating Dynamite on 28 realistic data migration scenarios.

==> fig-rules-attrmap.tex <==
\begin{figure}[!t]
\centering
\[
\small
\begin{array}{c}
\irulelabel
{\begin{array}{c}
    \attr \in \emph{Attrs}(\schema) \quad \attr' \in \emph{Attrs}(\schema') \\
    \emph{Values}(\eout, \attr') \subseteq \emph{Values}(\ein, \attr) \\
\end{array}}
{\schema, \schema', \ex \vdash \attr' \in \attrMap(\attr)}
{\textrm{(STMap)}} \\ \ \\

\irulelabel
{\begin{array}{c}
    \attr_1, \attr_2 \in \emph{Attrs}(\schema) \\
    \emph{Values}(\ein, \attr_2) \subseteq \emph{Values}(\ein, \attr_1) \\
\end{array}}
{\schema, \schema', \ex \vdash \attr_2 \in \attrMap(\attr_1)}
{\textrm{(SSMap)}} \\ \ \\

\end{array}
\]
\vspace{-10pt}
\caption{Rules for inferring the attribute mapping $\attrMap$ given source schema $\schema$, target schema $\schema'$, and example $\ex = (\ein, \eout)$. The function $\emph{Attrs}(x)$ returns all primitive attributes of schema $x$, and function $\emph{Values}(y, z)$ returns the set of values of attribute $z$ in instance $y$.}
\label{fig:rules-attrmap}
\end{figure}


==> fig-syntax-schema.tex <==
\begin{figure}[!t]
\centering
\[
\begin{array}{rcl}
\emph{Schema} \ \schema &::=& N \rightarrow T \\
\emph{Type} \ T &::=& \tau \ | \ \{ N_1, \ldots, N_n \} \\
\end{array}
\]
\caption{Syntax for representing database schemas. $N$ denotes the name of a record  type and $\tau $ is a primitive type}
\vspace{-10pt}
\label{fig:syntax-schema}
\end{figure}

